Bottlenecks in Blockchain Consensus Protocols

Most of the Blockchain permissioned systems employ Byzantine fault-tolerance (BFT) consensus protocols to ensure that honest validators agree on the order for appending entries to their ledgers. In this paper, we study the performance and the scalability of prominent consensus protocols, namely PBFT, Tendermint, HotStuff, and Streamlet, both analytically via load formulas and practically via implementation and evaluation. Under identical conditions, we identify the bottlenecks of these consensus protocols and show that these protocols do not scale well as the number of validators increases. Our investigation points to the communication complexity as the culprit. Even when there is enough network bandwidth, the CPU cost of serialization and deserialization of the messages limits the throughput and increases the latency of the protocols. To alleviate the bottlenecks, the most useful techniques include reducing the communication complexity, rotating the hotspot of communications, and pipelining across consensus instances.

==> Leaderless.tex <==
\section{Leaderless Protocols}
\label{sec:back1}
Here we Avalanche~\cite{AVA}  family of BFT protocols as an example of leaderless protocols. In our evaluations we provide results from an implementation of Snowball to compare it with the leader-based BFT protocols that is of the focus of our paper. 


Avalanche family of consensus protocols consists of Slush, Snowflake, Snowball, and Avalanche. These protocols provide strong probabilistic safety guarantee and guarantee liveness for correct client. They assume a synchronous network and use gossip algorithms to communicate between nodes. They employ a metastability mechanism and use tunable security parameters to make the possibility of a consensus failure arbitrarily small. This is achieved through the formation of sub-quorums, which are small, randomized samples from nodes on the network. Avalanche transactions confirm quicker than Nakamoto consensus and the protocols are faster and more scalable.

% \subsubsection{The Protocol}
% Avalanche-Snowball protocol as illustrated in Figure~\ref{fig:AVA} has four sub-protocols. The system operates by repeatedly sampling the participants at random, and steering the correct nodes towards the same consensus outcome.

In Slush, a node starts out initially in an uncolored state. Upon receiving a transaction from a client, an uncolored node updates its own color to the one carried in the transaction and initiates a query by picking a small, constant-sized ($k$) sample of the network uniformly at random, and sending a query message. Upon receiving a query, a colored node simply responds with its current color. On the other hand, an uncolored node adopts the color in the query and responds with that color, and initiates its own query. Once the querying node collects $k$ responses, it checks if a threshold fraction are for the same color. If this threshold (a configurable protocol parameter) is met and the sampled color differs from the node’s own color, the node flips to that color. The node then goes back to the query step, and initiates a subsequent round of query, for a total of m rounds. Finally, the querying node decides the color it ended up with at time m.


Snowflake sub-protocol augments Slush with a single counter that captures the strength of a node's conviction in its current color. Snowball sub-protocol augments Snowflake with confidence counters that captures which color has more confidence than other. Snowball protocols is illustrated in Figure~\ref{fig:AVA}.

Avalanche augments Snowball with directed acyclic graph (DAG) that maintains all known transactions. The use of DAGs in Avalanche enables storing blocks in a more concurrent and high-throughput way. 


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

